Neural Networks for Encoding Dynamic Security-Constrained Optimal Power Flow

This paper introduces a framework to capture previously intractable optimization constraints and transform them to a mixed-integer linear program, through the use of neural networks. We encode the feasible space of optimization problems characterized by both tractable and intractable constraints, e.g. differential equations, to a neural network. Leveraging an exact mixed-integer reformulation of neural networks, we solve mixed-integer linear programs that accurately approximate solutions to the originally intractable non-linear optimization problem. We apply our methods to the AC optimal power flow problem (AC-OPF), where directly including dynamic security constraints renders the AC-OPF intractable. Our proposed approach has the potential to be significantly more scalable than traditional approaches. We demonstrate our approach for power system operation considering N-1 security and small-signal stability, showing how it can efficiently obtain cost-optimal solutions which at the same time satisfy both static and dynamic security constraints.

==> Gen_dispatch.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
\definecolor{mycolor5}{rgb}{0.46600,0.67400,0.18800}%
%
\begin{tikzpicture}

\begin{axis}[%
width=8cm,
height=4cm,
xmin=1,
xmax=125,
xtick={1, 25, 50, 75, 100, 125},
ymin=20,
ymax=120,
xlabel={Instance of random cost function},
ylabel={Dispatch (MW)},
axis background/.style={fill=white},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot[const plot, color=mycolor1, line width=1pt] table[row sep=crcr] {%
1	108.012434440017\\
2	92.9054564755779\\
3	108.012434440017\\
4	102.113505828018\\
5	92.9054564755779\\
6	102.113505829889\\
7	108.012434440017\\
8	92.9054564755779\\
9	92.9054564755779\\
10	108.012434440017\\
11	110.936030193492\\
12	92.9054564755779\\
13	110.952011544843\\
14	92.9054564755779\\
15	110.952011544843\\
16	108.012434440017\\
17	108.012434440017\\
18	108.012434440017\\
19	92.9054564755779\\
20	92.9054564755779\\
21	92.9054564755779\\
22	92.9054564755779\\
23	92.9054564755779\\
24	92.9054564755779\\
25	102.113505828018\\
26	110.03185079884\\
27	92.9054564755779\\
28	110.936030193492\\
29	92.9054564755779\\
30	108.012434440017\\
31	107.902779167875\\
32	92.9054564755779\\
33	108.012434440017\\
34	108.012434440017\\
35	108.01243444007\\
36	110.936030193492\\
37	102.113505828018\\
38	108.012434440017\\
39	108.012434440017\\
40	108.012439434576\\
41	110.952011544843\\
42	102.113505828018\\
43	92.9054564755779\\
44	110.936030193492\\
45	92.9054564755779\\
46	110.952011544843\\
47	92.9054564755779\\
48	102.113505828018\\
49	108.012434440017\\
50	110.952011544843\\
51	110.952011544843\\
52	110.936030193492\\
53	92.9054564755779\\
54	110.936030193492\\
55	108.012434440017\\
56	110.952011544843\\
57	102.113505828018\\
58	110.936030193492\\
59	108.012434440017\\
60	92.9054564755779\\
61	92.9054564755779\\
62	108.012434440017\\
63	110.952011544843\\
64	108.012434440017\\
65	110.952011544843\\
66	102.113505828018\\
67	92.9054564755779\\
68	108.012434440017\\
69	108.012434440017\\
70	92.9054564755779\\
71	108.012434440017\\
72	102.113505828018\\
73	102.113505828018\\
74	110.936030193492\\
75	102.113505828018\\
76	92.9054564755779\\
77	102.113505828018\\
78	102.113505828019\\
79	102.113505828018\\
80	102.113505828018\\
81	92.9054564755779\\
82	92.9054564755779\\
83	92.9054564755779\\
84	110.936030193492\\
85	92.9054564755779\\
86	110.952011544843\\
87	108.012434440017\\
88	108.012434440017\\
89	110.952011544844\\
90	102.113505828019\\
91	108.012434440017\\
92	102.113505828018\\
93	102.113505828018\\
94	108.012434440017\\
95	92.9054564755779\\
96	108.012434440017\\
97	110.952011544844\\
98	102.113505828018\\
99	102.113505828018\\
100	92.9054564755779\\
101	108.012434440017\\
102	102.113505828018\\
103	108.012434440017\\
104	108.012440591245\\
105	92.9054564755779\\
106	92.9054564755779\\
107	92.9054564755779\\
108	92.9054564755779\\
109	92.9054564755779\\
110	92.9054564755779\\
111	102.113505828018\\
112	92.9054564755779\\
113	102.113505828018\\
114	92.9054564755779\\
115	92.9054564755779\\
116	92.9054564755779\\
117	102.113505828018\\
118	110.031850798841\\
119	92.9054564755779\\
120	102.113505828018\\
121	102.113505828019\\
122	92.9054564755779\\
123	102.113505828018\\
124	92.9054564755779\\
125	110.936030193492\\
};
%\addlegendentry{G1}

\addplot[const plot, color=mycolor2, line width=1pt] table[row sep=crcr] {%
1	45.188398879627\\
2	60\\
3	45.188398879627\\
4	60\\
5	60\\
6	60\\
7	45.188398879627\\
8	60\\
9	60\\
10	45.188398879627\\
11	46.692146145429\\
12	60\\
13	49.0318365191101\\
14	60\\
15	49.0318365191101\\
16	45.188398879627\\
17	45.188398879627\\
18	45.1883988796269\\
19	60\\
20	60\\
21	60\\
22	60\\
23	60\\
24	60\\
25	60\\
26	46.1469519758064\\
27	60\\
28	46.6921461454291\\
29	60\\
30	45.188398879627\\
31	45.2958164194734\\
32	60\\
33	45.188398879627\\
34	45.188398879627\\
35	45.188398879627\\
36	46.6921461454291\\
37	60\\
38	45.188398879627\\
39	45.188398879627\\
40	45.1883939869913\\
41	49.0318365191101\\
42	60\\
43	60\\
44	46.6921461454291\\
45	60\\
46	49.0318365191101\\
47	60\\
48	60\\
49	45.188398879627\\
50	49.0318365191101\\
51	49.0318365191101\\
52	46.692146145429\\
53	60\\
54	46.6921461454291\\
55	45.188398879627\\
56	49.0318365191101\\
57	60\\
58	46.6921461454291\\
59	45.188398879627\\
60	60\\
61	60\\
62	45.188398879627\\
63	49.0318365191101\\
64	45.188398879627\\
65	49.0318365191101\\
66	60\\
67	60\\
68	45.1883988796269\\
69	45.188398879627\\
70	60\\
71	45.188398879627\\
72	60\\
73	60\\
74	46.6921461454291\\
75	60\\
76	60\\
77	60\\
78	60\\
79	60\\
80	60\\
81	60\\
82	60\\
83	60\\
84	46.6921461454291\\
85	60\\
86	49.0318365191101\\
87	45.188398879627\\
88	45.188398879627\\
89	49.0318365191101\\
90	60\\
91	45.188398879627\\
92	60\\
93	60\\
94	45.188398879627\\
95	60\\
96	45.188398879627\\
97	49.0318365191101\\
98	60\\
99	60\\
100	60\\
101	45.188398879627\\
102	60\\
103	45.188398879627\\
104	45.1883928539268\\
105	60\\
106	60\\
107	60\\
108	60\\
109	60\\
110	60\\
111	60\\
112	60\\
113	60\\
114	60\\
115	60\\
116	60\\
117	60\\
118	46.1469519758064\\
119	60\\
120	60\\
121	60\\
122	60\\
123	60\\
124	60\\
125	46.6921461454291\\
};
%\addlegendentry{G2}

\addplot[const plot, color=mycolor3, line width=1pt] table[row sep=crcr] {%
1	60\\
2	60\\
3	60\\
4	51.2613954561917\\
5	60\\
6	51.2613954561916\\
7	60\\
8	60\\
9	60\\
10	60\\
11	55.7728820260521\\
12	60\\
13	53.4970007607654\\
14	60\\
15	53.4970007607654\\
16	60\\
17	60\\
18	60\\
19	60\\
20	60\\
21	60\\
22	60\\
23	60\\
24	60\\
25	51.2613954561916\\
26	57.1570323198088\\
27	60\\
28	55.7728820260521\\
29	60\\
30	60\\
31	60\\
32	60\\
33	60\\
34	60\\
35	60\\
36	55.7728820260521\\
37	51.2613954561916\\
38	60\\
39	60\\
40	60\\
41	53.4970007607654\\
42	51.2613954561917\\
43	60\\
44	55.7728820260521\\
45	60\\
46	53.4970007607654\\
47	60\\
48	51.2613954561916\\
49	60\\
50	53.4970007607654\\
51	53.4970007607654\\
52	55.7728820260521\\
53	60\\
54	55.7728820260521\\
55	60\\
56	53.4970007607654\\
57	51.2613954561916\\
58	55.7728820260521\\
59	60\\
60	60\\
61	60\\
62	60\\
63	53.4970007607654\\
64	60\\
65	53.4970007607654\\
66	51.2613954561917\\
67	60\\
68	60\\
69	60\\
70	60\\
71	60\\
72	51.2613954561917\\
73	51.2613954561916\\
74	55.7728820260521\\
75	51.2613954561916\\
76	60\\
77	51.2613954561916\\
78	51.2613954561917\\
79	51.2613954561917\\
80	51.2613954561917\\
81	60\\
82	60\\
83	60\\
84	55.7728820260521\\
85	60\\
86	53.4970007607654\\
87	60\\
88	60\\
89	53.4970007607654\\
90	51.2613954561916\\
91	60\\
92	51.2613954561917\\
93	51.2613954561917\\
94	60\\
95	60\\
96	60\\
97	53.4970007607654\\
98	51.2613954561916\\
99	51.2613954561917\\
100	60\\
101	60\\
102	51.2613954561917\\
103	60\\
104	60\\
105	60\\
106	60\\
107	60\\
108	60\\
109	60\\
110	60\\
111	51.2613954561916\\
112	60\\
113	51.2613954561917\\
114	60\\
115	60\\
116	60\\
117	51.2613954561917\\
118	57.1570323198089\\
119	60\\
120	51.2613954561917\\
121	51.2613954561916\\
122	60\\
123	51.2613954561917\\
124	60\\
125	55.7728820260521\\
};
%\addlegendentry{G3}

\addplot[const plot, color=mycolor4, line width=1pt] table[row sep=crcr] {%
1	25\\
2	25\\
3	25\\
4	25\\
5	25\\
6	25\\
7	25\\
8	25\\
9	25\\
10	25\\
11	25\\
12	25\\
13	25\\
14	25\\
15	25\\
16	25\\
17	25\\
18	25\\
19	25\\
20	25\\
21	25\\
22	25\\
23	25\\
24	25\\
25	25\\
26	25\\
27	25\\
28	25\\
29	25\\
30	25\\
31	25\\
32	25\\
33	25\\
34	25\\
35	25\\
36	25\\
37	25\\
38	25\\
39	25\\
40	25\\
41	25\\
42	25\\
43	25\\
44	25\\
45	25\\
46	25\\
47	25\\
48	25\\
49	25\\
50	25\\
51	25\\
52	25\\
53	25\\
54	25\\
55	25\\
56	25\\
57	25\\
58	25\\
59	25\\
60	25\\
61	25\\
62	25\\
63	25\\
64	25\\
65	25\\
66	25\\
67	25\\
68	25\\
69	25\\
70	25\\
71	25\\
72	25\\
73	25\\
74	25\\
75	25\\
76	25\\
77	25\\
78	25\\
79	25\\
80	25\\
81	25\\
82	25\\
83	25\\
84	25\\
85	25\\
86	25\\
87	25\\
88	25\\
89	25\\
90	25\\
91	25\\
92	25\\
93	25\\
94	25\\
95	25\\
96	25\\
97	25\\
98	25\\
99	25\\
100	25\\
101	25\\
102	25\\
103	25\\
104	25\\
105	25\\
106	25\\
107	25\\
108	25\\
109	25\\
110	25\\
111	25\\
112	25\\
113	25\\
114	25\\
115	25\\
116	25\\
117	25\\
118	25\\
119	25\\
120	25\\
121	25\\
122	25\\
123	25\\
124	25\\
125	25\\
};
%\addlegendentry{G4}



\end{axis}
\end{tikzpicture}%

\vspace{-0.15cm}
    \begin{center}
			         \begin{tikzpicture}
    \begin{axis}[%
    hide axis,
    xmin=1,
    xmax=2,
    ymin=0,
    ymax=0.1,
    legend style={draw=white!15!black,legend cell align=left},
    legend columns=5
    ]
    \addlegendimage{const plot, color=mycolor1, line width=1pt}
    \addlegendentry{Gen 1 \,};
    \addlegendimage{const plot, color=mycolor2, line width=1pt}
    \addlegendentry{Gen 2 \,};
        \addlegendimage{const plot, color=mycolor3, line width=1pt}
    \addlegendentry{Gen 3 \,};
        \addlegendimage{const plot, color=mycolor4, line width=1pt}
    \addlegendentry{Gen 4 and Gen 5\,};
    
    \end{axis}
    \end{tikzpicture}
     \end{center}
     



==> NN_1.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
%
\begin{tikzpicture}

\begin{axis}[%
width=8cm,
height=3cm,
xmin=0,
xmax=10,
ymin=99,
ymax=100,
ytick = {99,99.5,100},
ylabel={(\%)},
xlabel = {$\epsilon$},
axis background/.style={fill=white},
legend style={legend cell align=left, align=left, draw=white!15!black},
legend pos=outer north east
]

\addplot [color=mycolor2,line width = 1pt]
  table[row sep=crcr]{%
0	99.2875683437345\\
0.1	99.3695736326937\\
0.2	99.4354347705762\\
0.3	99.501329787234\\
0.4	99.5675076240643\\
0.5	99.6226205671791\\
0.6	99.6778493668074\\
0.7	99.7054573746804\\
0.8	99.7497636656843\\
0.9	99.7773944014692\\
1	99.8217865894408\\
1.1	99.8439937597504\\
1.2	99.8662207357859\\
1.3	99.888455103179\\
1.4	99.910719267898\\
1.5	99.9218488333147\\
1.6	99.9330020657696\\
1.7	99.944143439647\\
1.8	99.9552997709113\\
1.9	99.9608785558598\\
2	99.9720498630443\\
2.1	99.9720451749972\\
2.2	99.9832224148538\\
2.3	99.9832205380614\\
2.4	99.9888118147237\\
2.5	99.9888099367761\\
2.6	99.994404029099\\
2.7	99.9944034027311\\
2.8	100\\
2.9	100\\
3	100\\
3.1	100\\
3.2	100\\
3.3	100\\
3.4	100\\
3.5	100\\
3.6	100\\
3.7	100\\
3.8	100\\
3.9	100\\
4	100\\
4.1	100\\
4.2	100\\
4.3	100\\
4.4	100\\
4.5	100\\
4.6	100\\
4.7	100\\
4.8	100\\
4.9	100\\
5	100\\
5.1	100\\
5.2	100\\
5.3	100\\
5.4	100\\
5.5	100\\
5.6	100\\
5.7	100\\
5.8	100\\
5.9	100\\
6	100\\
6.1	100\\
6.2	100\\
6.3	100\\
6.4	100\\
6.5	100\\
6.6	100\\
6.7	100\\
6.8	100\\
6.9	100\\
7	100\\
7.1	100\\
7.2	100\\
7.3	100\\
7.4	100\\
7.5	100\\
7.6	100\\
7.7	100\\
7.8	100\\
7.9	100\\
8	100\\
8.1	100\\
8.2	100\\
8.3	100\\
8.4	100\\
8.5	100\\
8.6	100\\
8.7	100\\
8.8	100\\
8.9	100\\
9	100\\
9.1	100\\
9.2	100\\
9.3	100\\
9.4	100\\
9.5	100\\
9.6	100\\
9.7	100\\
9.8	100\\
9.9	100\\
10	100\\
};
%\addlegendentry{TNR}


\end{axis}


\end{tikzpicture}%

==> NN_2.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
%
\begin{tikzpicture}

\begin{axis}[%
width=8cm,
height=3cm,
xmin=0,
xmax=10,
ymin=85,
ymax=100,
ylabel={(\%)},
xlabel={$\epsilon$},
axis background/.style={fill=white},
legend style={legend cell align=left, align=left, draw=white!15!black},
legend pos=outer north east
]
\addplot [color=mycolor1, line width = 1pt]
  table[row sep=crcr]{%
0	99.3940903054449\\
0.1	99.4106905710491\\
0.2	99.4328242585215\\
0.3	99.4466578131917\\
0.4	99.4770916334661\\
0.5	99.4881584772023\\
0.6	99.5019920318725\\
0.7	99.5019920318725\\
0.8	99.5158255865427\\
0.9	99.5047587428066\\
1	99.5130588756087\\
1.1	99.5130588756087\\
1.2	99.5130588756087\\
1.3	99.5075254537406\\
1.4	99.5047587428066\\
1.5	99.4964586100044\\
1.6	99.4992253209385\\
1.7	99.4881584772023\\
1.8	99.4826250553342\\
1.9	99.4770916334661\\
2	99.4770916334661\\
2.1	99.468791500664\\
2.2	99.46602478973\\
2.3	99.4604913678619\\
2.4	99.4577246569279\\
2.5	99.4494245241257\\
2.6	99.4466578131917\\
2.7	99.4411243913236\\
2.8	99.4438911022576\\
2.9	99.4383576803896\\
3	99.4355909694555\\
3.1	99.4300575475874\\
3.2	99.4272908366534\\
3.3	99.4189907038513\\
3.4	99.4079238601151\\
3.5	99.4051571491811\\
3.6	99.3940903054449\\
3.7	99.3802567507747\\
3.8	99.3664231961045\\
3.9	99.3498229305002\\
4	99.333222664896\\
4.1	99.3000221336875\\
4.2	99.2640548915449\\
4.3	99.2363877822045\\
4.4	99.1865869853918\\
4.5	99.1284860557769\\
4.6	99.0648517042939\\
4.7	98.9929172200089\\
4.8	98.9154493138557\\
4.9	98.8213811420983\\
5	98.7162461266047\\
5.1	98.602810978309\\
5.2	98.4783089862771\\
5.3	98.339973439575\\
5.4	98.1905710491368\\
5.5	98.0245683930943\\
5.6	97.872399291722\\
5.7	97.6980965028774\\
5.8	97.5071934484285\\
5.9	97.3079902611775\\
6	97.1226206285967\\
6.1	96.9261841522798\\
6.2	96.7186808322266\\
6.3	96.5084108012395\\
6.4	96.3036741921204\\
6.5	96.1017042939354\\
6.6	95.880367419212\\
6.7	95.678397521027\\
6.8	95.479194333776\\
6.9	95.2661575918548\\
7	95.0697211155379\\
7.1	94.8732846392209\\
7.2	94.6713147410359\\
7.3	94.4887118193891\\
7.4	94.281208499336\\
7.5	94.1262726870297\\
7.6	93.9353696325808\\
7.7	93.7638335546702\\
7.8	93.6254980079681\\
7.9	93.4484285081895\\
8	93.3128596724214\\
8.1	93.1772908366534\\
8.2	93.0527888446215\\
8.3	92.953187250996\\
8.4	92.8342186808322\\
8.5	92.7678176184152\\
8.6	92.6709827357238\\
8.7	92.6073483842408\\
8.8	92.554780876494\\
8.9	92.4939132359451\\
9	92.4551792828685\\
9.1	92.4053784860558\\
9.2	92.3832447985834\\
9.3	92.3611111111111\\
9.4	92.3362107127047\\
9.5	92.3279105799026\\
9.6	92.3113103142984\\
9.7	92.3057768924303\\
9.8	92.3030101814962\\
9.9	92.2947100486941\\
10	92.2947100486941\\
};
%\addlegendentry{Accuracy}


\addplot [color=mycolor3,, line width = 1pt]
  table[row sep=crcr]{%
0	99.5010256694572\\
0.1	99.4518575937102\\
0.2	99.4302151905737\\
0.3	99.3921308576481\\
0.4	99.3870451156883\\
0.5	99.3544827586207\\
0.6	99.3274531422271\\
0.7	99.3002754820937\\
0.8	99.2841803865426\\
0.9	99.2352132049519\\
1	99.2082691884759\\
1.1	99.1866344251484\\
1.2	99.1650186772138\\
1.3	99.1325354123202\\
1.4	99.105525983647\\
1.5	99.0784421283598\\
1.6	99.0731091976087\\
1.7	99.0406227728743\\
1.8	99.0190168246835\\
1.9	99.0027943674319\\
2	98.992056970693\\
2.1	98.975791433892\\
2.2	98.9596451842523\\
2.3	98.9488091979195\\
2.4	98.9380337201664\\
2.5	98.9217886267856\\
2.6	98.9110211229069\\
2.7	98.9001969796454\\
2.8	98.9002571537999\\
2.9	98.8894359647683\\
3	98.8840262582057\\
3.1	98.873208620501\\
3.2	98.8678006891648\\
3.3	98.8515804440556\\
3.4	98.8299617277201\\
3.5	98.8245585260511\\
3.6	98.8029516261274\\
3.7	98.775956284153\\
3.8	98.7489756897023\\
3.9	98.7166184260827\\
4	98.6842823606486\\
4.1	98.6196737410661\\
4.2	98.5497764693054\\
4.3	98.4960767218832\\
4.4	98.3995645073489\\
4.5	98.2872056984395\\
4.6	98.164440099924\\
4.7	98.0260303687636\\
4.8	97.877409573316\\
4.9	97.6975462112204\\
5	97.4973031283711\\
5.1	97.2821699585598\\
5.2	97.047138408676\\
5.3	96.7873206254016\\
5.4	96.5082754938601\\
5.5	96.2001064395955\\
5.6	95.9193420005306\\
5.7	95.5997461392003\\
5.8	95.2521473362492\\
5.9	94.8921203212767\\
6	94.5595312826951\\
6.1	94.2096210976182\\
6.2	93.8427992939466\\
6.3	93.473989037129\\
6.4	93.1176591798887\\
6.5	92.768796510136\\
6.6	92.3894709941222\\
6.7	92.046033200937\\
6.8	91.7097919837646\\
6.9	91.3529084752615\\
7	91.0262866351093\\
7.1	90.7019920718551\\
7.2	90.3709629037096\\
7.3	90.0737492525414\\
7.4	89.7383706498536\\
7.5	89.4895786920145\\
7.6	89.1849220446023\\
7.7	88.9129365469749\\
7.8	88.6947988223749\\
7.9	88.4171395030327\\
8	88.2057287854389\\
8.1	87.9953266478434\\
8.2	87.8029824646622\\
8.3	87.6497114871745\\
8.4	87.4673376560534\\
8.5	87.3658772353794\\
8.6	87.2183353437877\\
8.7	87.121650279545\\
8.8	87.0419415418693\\
8.9	86.9498292366155\\
9	86.8913137528241\\
9.1	86.816195187551\\
9.2	86.7828508329733\\
9.3	86.7495320823535\\
9.4	86.712079055934\\
9.5	86.6996018993717\\
9.6	86.6746583553105\\
9.7	86.6663470297742\\
9.8	86.6621919647138\\
9.9	86.6497291596759\\
10	86.6497291596759\\
};
%\addlegendentry{TPR}


\end{axis}


\end{tikzpicture}%

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************

